Closed-loop Performance Optimization of Model Predictive Control with Robustness Guarantees

Model mismatch and process noise are two frequently occurring phenomena that can drastically affect the performance of model predictive control (MPC) in practical applications. We propose a principled way to tune the cost function and the constraints of linear MPC schemes to improve the closed-loop performance and robust constraint satisfaction on uncertain nonlinear dynamics with additive noise. The tuning is performed using a novel MPC tuning algorithm based on backpropagation developed in our earlier work. Using the scenario approach, we provide probabilistic bounds on the likelihood of closed-loop constraint violation over a finite horizon. We showcase the effectiveness of the proposed method on linear and nonlinear simulation examples.

==> Sources/header.tex <==
% Commands required by IEEE template
\IEEEoverridecommandlockouts
\overrideIEEEmargins

% References
\usepackage{csquotes}
\usepackage[english]{babel}

% Algorithms
\RequirePackage{algorithm,algpseudocode}
\algnewcommand\algorithmicinit{\textbf{Init:}}
\algnewcommand\Init{\item[\algorithmicinit]}
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}

% tables
\usepackage{booktabs}
\usepackage{multirow}

% Math packages
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{dsfont}
% \let\proof\relax
% \let\endproof\relax
% \usepackage{amsthm}

% Fonts
\let\Bbbk\relax
\usepackage[cmintegrals,cmbraces,varbb]{newtxmath} % Math font
\usepackage[cal=cm,bb=ams]{mathalpha} % Improve calligraphic and bb math
\renewcommand{\ttfamily}{\fontencoding{T1}\fontfamily{lmtt}\selectfont}

% Additional math options
\usepackage{xspace}

% Figures
\usepackage{graphicx}
\usepackage{caption}

% Captions of tables
\DeclareCaptionLabelFormat{mytablecaption}{#1 #2}
\captionsetup[table]{labelfont={it,small},labelformat=mytablecaption,labelsep=colon,font=small}
\captionsetup[figure]{labelfont={it,small},labelformat=mytablecaption,labelsep=colon,font=small}

% theorems
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{lemma}{Lemma}
\newtheorem{example}{Example}
% \theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}

% Math commands
\DeclareMathOperator*{\argmin}{arg\,min}

% Project-specific definitions
\newcommand{\Rpp}{\R_{>0}}
\newcommand{\Np}{\N_{>0}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rx}{\mathbb{R}^{n_x}}
\newcommand{\Rp}{\mathbb{R}^{n_p}}
\newcommand{\Rn}{\mathbb{R}^{n}}
\newcommand{\Ru}{\mathbb{R}^{n_u}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\PPP}{\mathscr{Y}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\J}{\mathcal{J}}
\renewcommand{\L}{\mathscr{L}}
\newcommand{\p}{\bar{p}}
\newcommand{\PP}{\mathscr{P}}
\newcommand{\mpc}{\mathrm{MPC}}
\newcommand{\tto}{\rightrightarrows}

\renewcommand{\P}{\mathscr{P}}

\usepackage{xcolor}
\definecolor{mycyan}{RGB}{0,113,188}
\newcommand{\eb}[1]{#1}
\newcommand{\rz}[1]{#1}
% \newcommand{\eb}[1]{\textcolor{red}{#1}}
\ifreview
    \newcommand{\rzz}[1]{\textcolor{mycyan}{#1}}
\else
    \newcommand{\rzz}[1]{#1}
\fi

% Hyperlinks and referencing
\makeatletter
\let\NAT@parse\undefined
\makeatother
\usepackage[hidelinks]{hyperref}
\usepackage[sort]{cleveref}

% Clever ref names
\crefname{appendix}{Appendix}{Appendices}
\AtBeginEnvironment{appendices}{\crefalias{section}{appendix}}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{theorem}{Theorem}{Theorems}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{section}{Section}{Sections}
\crefname{proposition}{Proposition}{Propositions}
\crefname{equation}{}{}
\crefmultiformat{equation}{(#2#1#3}{, #2#1#3)}{, #2#1#3}{, #2#1#3)}
\crefrangeformat{equation}{(#3#1#4-#5#2#6)}
\crefrangeformat{assumption}{Assumptions #3#1#4-#5#2#6}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{subsection}{Section}{Sections}
\crefname{paragraph}{Paragraph}{Paragraph}
\crefname{figure}{Figure}{Figures}
\crefname{table}{Table}{Tables}
\crefname{remark}{Remark}{Remark}
\crefname{table}{Table}{Table}
\crefname{definition}{Definition}{Definitions}

% Add vertical lines in algorithms
\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usepgfplotslibrary{groupplots}
\usepackage{hf-tikz}
\usetikzlibrary{tikzmark}
\usetikzlibrary{spy}
\usetikzlibrary{calc}
\usepackage{etoolbox}
\errorcontextlines\maxdimen
% begin vertical rule patch for algorithmicx (http://tex.stackexchange.com/questions/144840/vertical-loop-block-lines-in-algorithmicx-with-noend-option)
% note that some of the packages above are also needed
\newcommand{\ALGtikzmarkcolor}{black}% customise this, if you want
\newcommand{\ALGtikzmarkextraindent}{4pt}% customise this, if you want
\newcommand{\ALGtikzmarkverticaloffsetstart}{-.75ex}% customise this, if you want
\newcommand{\ALGtikzmarkverticaloffsetend}{-.5ex}% customise this, if you want
\makeatletter
\newcounter{ALG@tikzmark@tempcnta}
\newcommand\ALG@tikzmark@start{%
    \global\let\ALG@tikzmark@last\ALG@tikzmark@starttext%
    \expandafter\edef\csname ALG@tikzmark@\theALG@nested\endcsname{\theALG@tikzmark@tempcnta}%
    \tikzmark{ALG@tikzmark@start@\csname ALG@tikzmark@\theALG@nested\endcsname}%
    \addtocounter{ALG@tikzmark@tempcnta}{1}%
}
\def\ALG@tikzmark@starttext{start}
\newcommand\ALG@tikzmark@end{%
    \ifx\ALG@tikzmark@last\ALG@tikzmark@starttext
        % ignore this, the block was opened then closed directly without any other blocks in between (so just a \State basically)
        % don't draw a vertical line here
    \else
        \tikzmark{ALG@tikzmark@end@\csname ALG@tikzmark@\theALG@nested\endcsname}%
        \tikz[overlay,remember picture] \draw[\ALGtikzmarkcolor] let \p{S}=($(pic cs:ALG@tikzmark@start@\csname ALG@tikzmark@\theALG@nested\endcsname)+(\ALGtikzmarkextraindent,\ALGtikzmarkverticaloffsetstart)$), \p{E}=($(pic cs:ALG@tikzmark@end@\csname ALG@tikzmark@\theALG@nested\endcsname)+(\ALGtikzmarkextraindent,\ALGtikzmarkverticaloffsetend)$) in (\x{S},\y{S})--(\x{S},\y{E});%
    \fi
    \gdef\ALG@tikzmark@last{end}%
}
% the following line injects our new tikzmarking code
\apptocmd{\ALG@beginblock}{\ALG@tikzmark@start}{}{\errmessage{failed to patch}}
\pretocmd{\ALG@endblock}{\ALG@tikzmark@end}{}{\errmessage{failed to patch}}
\makeatother
% end vertical rule patch for algorithmicx

\definecolor{myBlue}{RGB}{31,119,180}
